ShapeFlow: Learnable Deformations Among 3D Shapes

We present ShapeFlow, a flow-based model for learning a deformation space for entire classes of 3D shapes with large intra-class variations. ShapeFlow allows learning a multi-template deformation space that is agnostic to shape topology, yet preserves fine geometric details. Different from a generative space where a latent vector is directly decoded into a shape, a deformation space decodes a vector into a continuous flow that can advect a source shape towards a target. Such a space naturally allows the disentanglement of geometric style (coming from the source) and structural pose (conforming to the target). We parametrize the deformation between geometries as a learned continuous flow field via a neural network and show that such deformations can be guaranteed to have desirable properties, such as be bijectivity, freedom from self-intersections, or volume preservation. We illustrate the effectiveness of this learned deformation space for various downstream applications, including shape generation via deformation, geometric style transfer, unsupervised learning of a consistent parameterization for entire classes of shapes, and shape interpolation.

==> figures/canonical_tikz.tex <==
\begin{tikzpicture}[node distance=0em, auto]

\tikzset{>=latex}
\def\w{1.5cm}

\small

% original

\node (orig_0) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/src_0.png}}; %images go here
\node [left=-1em of orig_0,text width=5em] (orig_cap) {\textit{Original Shapes}};
\node [right=0em of orig_0] (orig_1) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/src_1.png}}; %images go here
\node [right=0em of orig_1] (orig_2) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/src_2.png}}; %images go here
\node [right=0em of orig_2] (orig_3) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/src_3.png}}; %images go here
\node [right=0em of orig_3] (orig_4) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/src_4.png}}; %images go here

% original

\node [below=0em of orig_0] (can_0) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/can_0.png}}; %images go here
\node [left=-1em of can_0,text width=5em] (can_cap) {\textit{Canonical Pose}};
\node [right=0em of can_0] (can_1) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/can_1.png}}; %images go here
\node [right=0em of can_1] (can_2) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/can_2.png}}; %images go here
\node [right=0em of can_2] (can_3) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/can_3.png}}; %images go here
\node [right=0em of can_3] (can_4) {\includegraphics[width=\w,height=\w,trim={0 0 0 0},clip]{figs/canonical/can_4.png}}; %images go here

\end{tikzpicture}

==> tables/canonical.tex <==
\begin{table}
\begin{tabular}{@{}ll@{}}
\toprule
                & Semantic \\
Matching        & Matching \\
Domain          & Score    \\ \midrule
Original        &          \\
Canonical       &          \\ \bottomrule
\end{tabular}%
\end{table}
